Analyzing the Forgetting Problem in the Pretrain-Finetuning of Dialogue Response Models

In this work, we study how the finetuning stage in the pretrain-finetune framework changes the behavior of a pretrained neural language generator. We focus on the transformer encoder-decoder model for the open-domain dialogue response generation task. Our major finding is that after standard finetuning, the model forgets some of the important language generation skills acquired during large-scale pretraining. We demonstrate the forgetting phenomenon through a set of detailed behavior analysis from the perspectives of knowledge transfer, context sensitivity, and function space projection. As a preliminary attempt to alleviate the forgetting problem, we propose an intuitive finetuning strategy named "mix-review". We find that mix-review effectively regularizes the finetuning process, and the forgetting problem is alleviated to some extent. Finally, we discuss interesting behavior of the resulting dialogue model and its implications.

==> eacl2021_rebuttal.tex <==
General:

We sincerely thank all reviewers for their insightful comments and suggestions! Please refer to our responses to individual reviewers.

Review#1

Thanks for the review! Here's our responses to your questions:

Re "how were the three prompts chosen for the dialogue and news style generation tasks?":

A: Sorry about the confusion. The six templates are manually chosen by us to reflect the nature of dialogue or news-style texts. We design them (shown in Table 3) to be "... about X", so that each knowledge term (e.g., pokemon or deadpool) can easily replace the "X" in the template. We will also clarify this in the manuscript.

Re "What is missing though is a section on when the mix-review method fails?":

A: Yes that's a very good suggestion. As we said in the manuscript, the mix-review is only a preliminary attempt to alleviate the forgetting problem, and there are indeed cases that the model trained by mix-review fails to give interesting output. We will add discussions/examples to the updated version of this manuscript. Thanks!

Re "there is a small section where the paper discusses the problem of generating malicious responses ... how often does this phenomenon occur?"：

A: Yes, that section is more of pointing out a future research direction than addressing it.  It does not usually occur. We pointed out that it can respond in a malicious way when we deliberately "provoke" it. 

Review#2

Thanks for the review! Here's our responses to your questions:

Re A1 "Not sure it is consistent with knowledge within the pretrained CCNEWS":

A: We explained in line 454-459 that we used Google trend data of 2016, and the CCNEWS data contains news in 2016. We manually checked that most of the knowledge terms indeed exist in the CCNEWS data. The intuition is that we expect the model to at least remember the biggest 2016 news from 2016. 

Re A2 "What’s more, I am also curious about news-trigger on dialog dataset, will a news-style trigger are more efficient to get a higher BLEU?":

A: Note that we use dialog trigger for the finetuned models. In our preliminary trials, we find that news trigger will give inferior BLEU scores. We believe the intuition is that the model is finetuned for dialogue datasets, afterall.

Re A4(also D3) "Is it because of adding more pretraining data with that knowledge or just because of the training objective":

A: We explained that (line 294) in mix-review we just randomly sample a tiny portion of the pretraining data, and we did not force it to contain any google trend knowledge. So, we believe the main reason is because of the training objective. As shown in Figure 2, this randomly sampled data is enough to effectively make the model retain its performance on the pretraining data.

Re B1 "The results on Cornell in the appendix seems not significant.":

A: Table 10 shows that the sensitivity from mix-review is larger than the fine-tuned baseline by a meaningful margin.

Re D1 "beside the Table 2, maybe a human evaluation will be better to compare how different fine-tuning strategies on the target task.":

A: We have a human evaluation of knowledgeable dialogue in Table 5, and mix-review gives meaningful improvements.

Re D2 "equation 3, do we consider all the parameters including the embedding?"

A: Yes, all parameters are included. We find that a large lambda such as 0.1 or 0.01 for weight decay works best.

Re D3 "what is the best hyper-parameter for Table 2. ":

A: We explained in line 317 that the performance of mix-review is not sensitive to hyper-parameter tuning. A small mix-ratio of 4 works well. Please also refer to our answer of A4.

Re typos and references

Thanks for pointing those out! We will fix them and add the reference into the manuscript. Regarding Table 3, you can replace "pokemon" with "deadpool" in the triggers. We will also clarify this in the updated manuscript.

Review#3

Thanks for the review! Here's our responses to your questions:

Re "What is the definition of the forgetting problem, and how to quantify the degree of forgetting?"

A: In this work we have designed several experiments to quantify the degree of forgetting. For example, in Section 5.1 (knowledge transfer), we check how much information related to the knowledge terms the model can remember, by comparing its generation to the reference description.  We then quantify the degree of forgetting by comparing the BLEU score of the fine-tuned model to the pretrained model's BLEU score.

Review#4

Thanks for the review!



==> mix_train.tex <==
\vspace{-0.1cm}
\subsection{Mix-train: a Low-cost Alternative for the Pretrain-Finetune Framework}
\label{sec:mixtrain_exp}
\vspace{-0.1cm}

In this section, we explore the \textit{mix-train} strategy, which is essentially the same procedure as mix-review, but starts from random initialization, instead of the pre-trained model. In particular, we compare it to the standard pretrain-finetune framework, and find it to be an attractive low-cost alternative.

Mix-train shares the same hyper-parameters with mix-review, namely mix-ratio and mix-decay. We tune the hyper-parameters in the grid of $\{4, 8, 16, 32, 64, 128, 256\} \bigtimes \{1, 0.95, 0.9, 0.85, 0.8, 0.75\}$ based on the PPL performance on the target dialogue validation set. We use 8 GPUs for each mix-train experiment, other hyper-parameters (e.g. learning rate or batch size) are kept the same with the standard pre-training experiments.

The resulting PPL and computational cost in terms of GPU-hour (GPUh) is shown in Table \ref{tab:mixtrain_main}. We show two configurations of mix-ratio, resulting in two different amounts of computing resources. We find that mix-train achieves significantly better performance compared to the standard pretrain-finetuning with the same amount of computing resources, and comes close to the performance of full-scale pretrain-finetune procedure. This shows that mix-train is a more effective way of utilizing the large-scale pre-training data when the computing resources are limited.

%, so that the computational resources used (for each experiment) is less than 10\% of the resources used for the standard pretrain-finetuning.

\begin{table}[]
\centering
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
            & \multicolumn{2}{c|}{\bf Dailydialogue} & \multicolumn{2}{c|}{\bf Switchboard} & \multicolumn{2}{c|}{\bf Cornell} \\ \hline
Model       & PPL            & Computing         & PPL           & Computing        & PPL         & Computing      \\ \hline
Baseline    & 24.83          &    8GPUh               & 51.14         &       4GPUh      & 49.48       &     10GPUh         \\ \hline
Mix-train(1)   & 12.44          & 128GPUh           & 32.23         & 88GPUh           &    36.44 & 121GPUh    \\ \hline
Partial P-F(1) & 17.64         & 128GPUh           & 42.00         & 88GPUh           &    39.99 & 121GPUh      \\ \hline
Mix-train(2) & 12.09 & 228GPUh & 31.39  & 168GPUh & 30.46       &       435GPUh \\ \hline
Partial P-F(2) & 15.14 & 228GPUh & 35.84 & 168GPUh &  32.42  &   435GPUh   \\ \hline
Full P-F    & 11.54         & 5120GPUh          & 26.37         & 5120GPUh         & 26.37       & 5120GPUh       \\ \hline
\end{tabular}
\caption{Comparison of mix-train to baseline and the standard pretrain-finetune process (denoted as P-F). Note that for comparison with partial P-F, we first take the pre-training checkpoint with the same amount of GPUh of mix-train, and then fine-tune it.}
\label{tab:mixtrain_main}
\end{table}

In Figure \ref{fig:mixtrain_difftratio}, we analyze the performance pattern of mix-train with different mix-ratio and mix-decay. It is shown that when mix-ratio is relatively small (e.g. 8), the best performance is achieved without mix-decay. But when mix-ratio is set to a large value (e.g. 128), then mix-decay becomes important. The reason is that under large mix-ratio, the training can ignore the target dialogue data, and just focus on the pre-training CCNEWS data. And mix-decay is needed to shift the focus back. So in the large mix-ratio regime, the mix-train process is becoming more similar to the standard pretrain-finetune framework. As shown in Table \ref{tab:mixtrain_main}, the performance gain of mix-train diminishes as more computing resource is used.


==> zzz_iclr2020_rebutal.tex <==
HEAD
Paper change: 
(1) We add a multi-turn human knowledgeable dialogue evaluation in Table 7 (Section 5.3). It shows mix-review outperforms weight-decay significantly. It focus on whether the model remembers the knowledge existing in the pre-training news data, which is not well reflected in the evaluations in Section 5.1. We believe this evaluation is a better judgement of how well the training utilizes the pre-training data, and we hope reviewers can take this result into consideration. 
(2) We change the title to emphasis that we focus on identifying and analyzing the forgetting problem for pre-trained NLG models.

TAIL
We thank the reviewer again, and are willing to continue the helpful discussion.

Reviewer#1
(1) In Figure 1(a), it looks the line of mixreview_ccnews_valid does not change at all. Does this indicate the fine-tuning on a dialogue dataset, which should be different from the CCNEWS data, does not change the model's ability in generating CCNEWS at all? Can the authors give some more explanations here?

Answer: Re-taining the performance on CCNEWS is the effect of mix-review. As shown by the blue dotted line in Figure 1(a), without mix-review the performance on CCNEWS drops drastically, which matches our intuition.

(2) Raters are asked to give overall ratings on generated text in Table 2. While this human evaluation is great plus, readers may also like to see some finer-grained human analysis, such as human evaluations from different angles, such as cohere, fluency, engageness and so on. Such detailed evaluations can also better reveal why the mix-review strategy is working better.

Answer: Yes, we now provide these results in Table 12 in the Appendix. We also address this in Table 7.

(3) In Table 4 and Table 6, the NS and MASS pre-training tasks are utilized separately? Why not combine these tasks together? Will there be more gain of doing so?

Answer: In the beginning, we don't know which of MASS and NS is better for the end dialogue response task. Table 2 and Table 4 show that NS gives better PPL and context sensitivity. So we focus on NS pre-training for the mix-review experiments. Further, MASS pre-training will make our analysis in Section 5.2 difficult (it will be non-straightforward to trigger the MASS pre-trained model to output knowledge). Finally, pre-training is not the focus of this work.

(4) Table 3 is a great analysis. I'm wondering if it is possible to evaluate the context-sensitivity quantitatively?

Answer: We don't quite understand your question. We believe Table 4 is already a quantitative analysis. For qualitative examples, we provide some dialogue examples in Table 8 and Table 10, where you can observe that the model trained by mix-review can generate coherent responses.

(5) What do you mean by "trigger" in Sec. 5.3? Using the triggers as the input context to the generation model? What's the relationship between the reference description and the triggers? It seems the reference descriptions are some factual statements that are crawled independently with the triggers. 

Answer: Yes, we feed the trigger inputs to the model as context input, and collect output samples. "Trigger" means that we want to guide the model to give outputs relevant to a knowledge term. And yes, the descriptions are part of the Google Trend 2016, which are used to judge how much the models knows about the knowledge term. 


Reviewer#2
Q: The two analyses are also not convincing to show mix-review performs better. For example, in terms of context-sensitivity, the increase in perplexity after distort the context does not necessarily mean the model’s generation is more context-related.  
A: For knowledge transfer, we add a multi-turn human evaluation in Table 7, which convincingly shows that mix-review is better at conducting knowledgeable dialogues. The context sensitivity analysis is from the paper "Do Neural Dialog Systems Use the Conversation History Effectively? An Empirical Study.", which is accepted at ACL. In Table 12, it is shown that pre-trained model has significantly better consistency comparing to the model trained from scratch, which correlates well with the context sensitivity analysis. We are very willing to improve this measurement if you have more detailed advice. 

Q: It is not surprising using this strategy alleviates the forgetting problem, but the question is whether it can make the model generalize better.
A: Note that the pre-training data is non-dialogue news, while the fine-tuning data is dialogue data. So, simply retraining performance on the pre-training data won't necessarily help the end dialogue task (the situation here is more complicated than the standard continual learning case). We show that with mix-review, the model is able to transfer the news knowledge or context sensitivity into a dialogue setting, which is non-trivial.

Q: The proposed mix-review strategy is very straightforward and lacks novelty.
A: The major novelty of our work lies not in the proposition of the algorithm, but in analyzing the forgetting problem for pre-trained NLG models. Note that the forgetting problem here is not as clearly defined as in the continual learning case, because losing performance on the pre-training data is not necessarily bad. We focus on whether fine-tuning transfer some desirable generative properties to the end task, which is non-trivial to analyze. About the simplicity of our algorithm, we want to point out there are advantages for being simple: mix-review doesn't require modification to the transformer model or to the time-consuming pre-training process. Moreover, the effect of rehearsal-based methods has never been explored in the context of NLG model training.

Q: Contribution not big
A: We agree that in the standard continual learning context, we don't make a big contribution. Our contribution mainly lies in how we show the forgetting problem is different in the context of pre-trained NLG models, and provide principled ways to analyze it.

Reviewer #3
Q: The approach of the paper (Mix-Review) is very similar to methods that have been proposed already.
A: The major novelty of our work lies not in the proposition of the algorithm, but in analyzing the forgetting problem for pre-trained NLG models. Note that the forgetting problem here is not as clearly defined as in the continual learning case, because losing performance on the pre-training data is not necessarily bad. We focus on whether fine-tuning transfer some desirable generative properties to the end task, which is non-trivial to analyze. About the simplicity of our algorithm, we want to point out there are advantages for being simple: mix-review doesn't require modification to the transformer model or to the time-consuming pre-training process. Moreover, the effect of rehearsal-based methods has never been explored in the context of NLG model training.

Q: There is a small gain that seems to be within the confidence intervals (assuming that is what is shown in parentheses).
A: We add a multi-turn human knowledgeable dialogue evaluation in Table 7 (Section 5.3). For that evaluation, mix-review is shown to outperforms weight-decay significantly.

Q: figure 1 doesn’t tell us very much
A: Figure 1 mainly serves as a motivation demonstrating there seems to exist a serious forgetting issue during fine-tuning. Whether it really exists is answered by Section 5.2 and 5.3. It then shows that with a small mix-ratio, the performance on the pre-training data can be retained, which is non-trivial. It also shows mix-review alleviates over-fitting to some extent. 

Q: Now, the actual issue is that early stopping is NOT applied consistently between WD and mix-review, as the WD approach has seen the pretraining data only 20 times (“we stop the pre-training after the CCNEWS data is swept 20 time”), but mix-review continues to be shown CCNEWS data even after 20 epochs, so there is effectively no early stopping for mix-review.
A: Good question. Firstly, more epochs of pre-training won't help the forgetting problem during fine-tuning, so it won't change the results in Section 5.2 and 5.3. Moreover, we believe the additional pre-training data used during mix-review is not going to make a visible difference on PPL, the reason is that the fine-tuning is only run for a few epochs, and only a small mix-ratio is used. Take the Dailydialogue experiment for example, we calculate that  mix-review only uses 2\% of the pre-training data, which is negligible comparing to the computing (swept for 20 times) used in pre-training.

Q: give credit to Kirkpatrick [2017] 
A: Thanks, we added the citation to the paper.

Q: About the mix-decay parameter
A: We now add the mix-decay to Equation (2) for clarity. Your understanding of mix-decay is correct. We introduce mix-decay to enable us to try larger mix-ratio, however, we find that a small mix-ratio (e.g. less than 4) is enough to work well. An advantage of mix-review is that it is not sensitive to hyper-parameter tuning.
